A new foreperiod effect on single-trial phase coherence. Part I: existence and relevance

Expecting events in time leads to more efficient behavior. A remarkable early finding in the study of temporal expectancy is the foreperiod effect on reaction times; i.e., the influence or reaction time of the time period between a warning signal and an imperative stimulus to which subjects are instructed to respond as quickly as possible. Recently it has been shown that the phase of oscillatory activity preceding stimulus presentation is related to behavior. Here we connect both of these findings by reporting a novel foreperiod effect on the inter-trial phase coherence of the electroencephalogram (EEG) triggered by stimuli to which subjects are instructed not to respond. Inter-trial phase coherence has been used to describe regularities in phases of groups of trials time locked to an event of interest. We propose a single-trial measure of inter-trial phase coherence and prove its soundness. Equipped with this measure, and using a multivariate decoding method, we demonstrate that the foreperiod duration in and audiovisual attention-shifting task modulates single-trial phase coherence. In principle, this modulation could be an artifact of the decoding method used to detect it. We show that this is not the case, since the modulation can also be observed using a simple averaging method. We show that the strength of this modulation correlates with subject behavior (both error rates and mean-reaction times). We anticipate that the new foreperiod effect on inter-trial phase coherence, and the decoding method used here to detect it, will be important tools to understand cognition at the single-trial level. In Part II of this manuscript, we support this claim, by showing that changes in attention modulate the strength of the new foreperiod effect on a trial-by-trial basis.

==> tables/statsCorCoefsPeakITCsVsErrorRatesFilterByBootCITabular.tex <==
\begin{tabular}{|c|c|c|c|}\hline
\multicolumn{1}{|c}{C} & \multicolumn{1}{|c}{S}  & \multicolumn{1}{|c}{Switch Vision}  & \multicolumn{1}{|c|}{Switch Audition}\\ \hline \hline
03 & V & -0.36 (-0.77, 0.23) & 0.35 (-0.27, 0.76) \\
 & A & \cellcolor{Red}{-0.51 (-0.82, -0.01)} & 0.15 (-0.43, 0.66) \\
\hline
04 & V & \cellcolor{Red}{-0.53 (-0.82, -0.03)} & -0.14 (-0.64, 0.38) \\
 & A & 0.52 (-0.18, 0.92) & -0.32 (-0.72, 0.20) \\
\hline
05 & V & -0.36 (-0.79, 0.22) & 0.13 (-0.61, 0.75) \\
 & A & -0.24 (-0.79, 0.50) & -0.38 (-0.82, 0.35) \\
\hline
06 & V & 0.03 (-0.50, 0.51) & -0.01 (-0.60, 0.50) \\
 & A & -0.23 (-0.68, 0.31) & -0.35 (-0.76, 0.11) \\
\hline
07 & V & -0.49 (-0.97, 0.26) & 0.20 (-0.60, 0.70) \\
 & A & -0.39 (-0.87, 0.28) & -0.33 (-0.84, 0.62) \\
\hline
09 & V & 0.03 (-0.62, 0.70) & -0.34 (-0.80, 0.24) \\
 & A & \cellcolor{Red}{-0.62 (-0.96, -0.03)} & \cellcolor{Red}{-0.58 (-0.87, -0.07)} \\
\hline
10 & V & -0.38 (-0.88, 0.38) & 0.31 (-0.54, 0.89) \\
 & A & -0.13 (-0.73, 0.71) & -0.10 (-0.71, 0.54) \\
\hline
11 & V & 0.12 (-0.47, 0.72) & 0.08 (-0.56, 0.66) \\
 & A & \cellcolor{Red}{-0.69 (-0.93, -0.19)} & -0.29 (-0.84, 0.45) \\
\hline
13 & V & -0.24 (-0.77, 0.52) & \cellcolor{Red}{0.77 (0.34, 0.96)} \\
 & A & -0.34 (-0.88, 0.41) & \cellcolor{Red}{-0.72 (-0.97, -0.17)} \\
\hline
14 & V & \cellcolor{Red}{-0.50 (-0.77, -0.01)} & -0.39 (-0.85, 0.34) \\
 & A & -0.27 (-0.79, 0.42) & -0.31 (-0.91, 0.51) \\
\hline
15 & V & 0.25 (-0.30, 0.66) & -0.02 (-0.47, 0.50) \\
 & A & -0.35 (-0.96, 0.30) & \cellcolor{Red}{-0.54 (-0.81, -0.12)} \\
\hline
17 & V & -0.25 (-0.92, 0.59) & -0.06 (-0.83, 0.84) \\
 & A & 0.48 (-0.36, 1.00) & -0.02 (-0.84, 0.84) \\
\hline
18 & V & -0.34 (-0.86, 0.26) & -0.03 (-0.71, 0.64) \\
 & A & -0.21 (-0.64, 0.37) & \cellcolor{Red}{-0.67 (-0.92, -0.22)} \\
\hline
19 & V & 0.15 (-0.52, 0.76) & 0.18 (-0.57, 0.75) \\
 & A & -0.04 (-0.76, 0.65) & \cellcolor{Red}{-0.85 (-0.97, -0.50)} \\
\hline
\end{tabular}


==> tables/statsCorCoefsPeakITCsVsMeanRTsFilterByBootCITabular.tex <==
\begin{tabular}{|c|c|c|c|}\hline
\multicolumn{1}{|c}{C} & \multicolumn{1}{|c}{S}  & \multicolumn{1}{|c}{Switch Vision}  & \multicolumn{1}{|c|}{Switch Audition}\\ \hline \hline
03 & V & -0.22 (-0.64, 0.37) & 0.25 (-0.35, 0.72) \\
 & A & -0.46 (-0.81, 0.06) & -0.09 (-0.51, 0.40) \\
\hline
04 & V & -0.08 (-0.59, 0.51) & 0.00 (-0.53, 0.48) \\
 & A & 0.02 (-0.51, 0.53) & -0.28 (-0.73, 0.28) \\
\hline
05 & V & 0.15 (-0.39, 0.61) & 0.41 (-0.18, 0.73) \\
 & A & -0.06 (-0.59, 0.63) & -0.19 (-0.70, 0.42) \\
\hline
06 & V & -0.28 (-0.74, 0.25) & 0.00 (-0.55, 0.53) \\
 & A & -0.23 (-0.71, 0.30) & -0.33 (-0.69, 0.15) \\
\hline
07 & V & -0.04 (-0.74, 0.64) & 0.08 (-0.62, 0.66) \\
 & A & 0.05 (-0.72, 0.69) & 0.03 (-0.69, 0.82) \\
\hline
09 & V & -0.16 (-0.62, 0.41) & -0.05 (-0.62, 0.53) \\
 & A & 0.12 (-0.36, 0.57) & -0.31 (-0.72, 0.22) \\
\hline
10 & V & 0.19 (-0.72, 0.80) & 0.40 (-0.25, 0.88) \\
 & A & 0.39 (-0.40, 0.84) & -0.04 (-0.72, 0.55) \\
\hline
11 & V & -0.21 (-0.72, 0.40) & -0.17 (-0.79, 0.45) \\
 & A & -0.43 (-0.88, 0.20) & 0.26 (-0.39, 0.69) \\
\hline
13 & V & 0.25 (-0.44, 0.76) & 0.54 (-0.09, 0.90) \\
 & A & 0.09 (-0.59, 0.84) & -0.26 (-0.86, 0.49) \\
\hline
14 & V & -0.24 (-0.66, 0.35) & -0.17 (-0.64, 0.55) \\
 & A & -0.27 (-0.78, 0.42) & -0.22 (-0.69, 0.36) \\
\hline
15 & V & -0.23 (-0.59, 0.27) & -0.03 (-0.49, 0.43) \\
 & A & 0.03 (-0.44, 0.48) & -0.23 (-0.64, 0.28) \\
\hline
17 & V & -0.18 (-1.00, 0.65) & 0.06 (-0.91, 0.82) \\
 & A & -0.15 (-0.83, 0.62) & \cellcolor{Red}{-0.74 (-0.94, -0.13)} \\
\hline
18 & V & -0.31 (-0.74, 0.30) & \cellcolor{Red}{-0.58 (-0.88, -0.07)} \\
 & A & 0.15 (-0.44, 0.67) & -0.21 (-0.70, 0.43) \\
\hline
19 & V & -0.39 (-0.79, 0.20) & -0.02 (-0.54, 0.57) \\
 & A & -0.13 (-0.77, 0.47) & -0.17 (-0.67, 0.38) \\
\hline
\end{tabular}

